Unsupervised Anomaly Detection with Rejection

Anomaly detection aims at detecting unexpected behaviours in the data. Because anomaly detection is usually an unsupervised task, traditional anomaly detectors learn a decision boundary by employing heuristics based on intuitions, which are hard to verify in practice. This introduces some uncertainty, especially close to the decision boundary, that may reduce the user trust in the detector's predictions. A way to combat this is by allowing the detector to reject examples with high uncertainty (Learning to Reject). This requires employing a confidence metric that captures the distance to the decision boundary and setting a rejection threshold to reject low-confidence predictions. However, selecting a proper metric and setting the rejection threshold without labels are challenging tasks. In this paper, we solve these challenges by setting a constant rejection threshold on the stability metric computed by ExCeeD. Our insight relies on a theoretical analysis of such a metric. Moreover, setting a constant threshold results in strong guarantees: we estimate the test rejection rate, and derive a theoretical upper bound for both the rejection rate and the expected prediction cost. Experimentally, we show that our method outperforms some metric-based methods.

==> neurips_texfiles/theory.tex <==
\subsection{Theoretical Guarantees}\label{sec:methodology_theoretical_results}
\changed{Although introducing a reject option into a detector may have some risks. First, one would like to know beforehand the expected proportion of rejected predictions such that the detector does not end up rejecting all of them, which would make it useless in practice. Moreover, the risk of obtaining an excessive cost at prediction time can be a cause for doubting the model. Thus, we provide a theoretical answer to the following relevant questions:}
\begin{itemize}
    \item[R1.] Does \ourmethod{} always keep the rejection rate low?
    \item[R2.] Can we get an estimate of \ourmethod{}'s rejection rate?
    \item[R3.] Is the expected prediction cost by \ourmethod{} bounded?
\end{itemize}

\paragraph{R1. An upper bound for the rejection rate.}
\begin{definition}\label{defn:rejection_rate}
Given a confidence metric $\mathscr{C} \colon \R^d \to [0,1]$ and a rejection threshold $\tau \in [0,1]$, the \textbf{rejection rate $\mathcal{R}$} is the probability that an example $x$ gets confidence below $\tau$:
\begin{equation*}
    \mathcal{R} = \Pp_X(\mathscr{C}_x \le \tau).
\end{equation*}
\end{definition}
\begin{remark}
Using \exceed{} to estimate the model confidence, and setting $\tau = 1-e^{-T}$ for $T\ge 4$ yield to
$$\mathcal{R} = \Pp_X(\mathscr{C}_x \le \tau) = \Pp_S\left(\mathscr{C}(\hat{Y})_s \in \left[e^{-T}, 1- e^{-T}\right]\right).$$
\end{remark}
In the following theorem, we provide an upper bound for the rejection rate:
\begin{theorem}\label{thm:rejection_rate_bounded}
Let $\mathscr{C}(\hat{Y})_s$ be the confidence of $s\sim S$ for a detector $f$, and the rejection threshold be $\tau = 1 - e^{-T}$ for any $T\ge 4$. For $n\in\N$, $\gamma \in [0,0.5)$, and small $\delta>0$, there exists a positive real function $h(n,\gamma,T,\delta)$ such that $\mathcal{R} \le h(n,\gamma,T,\delta)$ with probability at least $1-\delta$, i.e. the rejection rate is bounded by $h$.
\end{theorem}
\begin{proof}
Theorem~\ref{thm:confidence_bounded} states that there exists two functions $t_1 = t_1(n,\gamma,T), t_2 = t_2(n,\gamma,T) \in [0,1]$ such that the confidence is lower than $\tau$ if $\psi_n \in [t_1,t_2]$. Note that if $t^*\in[0,1]$ is such that $\mathscr{C}(\hat{Y})_s = 0.5$ for $\psi_n = t^*$, then $\mathscr{C}(\hat{Y}=1)_s \le \tau$ for $\psi_n \in [t^*, t_2]$ and $\mathscr{C}(\hat{Y}=0)_s \le \tau$ for $\psi_n \in [t_1,t^*]$ (Corollary~\ref{cor:properties_confidence_bounds}, property P4). Measuring these two intervals is the same as measuring $[t_1,t_2]$. Moreover, when varying $s \sim S$, the variable $\psi_n$ has a distribution that is arbitrarily close to uniform: Theorem~\ref{thm:tau_is_uniform} shows that $\psi = F_S(S)$ has a uniform distribution $\psi \sim Unif(0,1)$, while Theorem~\ref{thm:empirical_tau} claims that $\psi_n$ has a distribution that is close to $\psi$ with high probability (see the theorems and proofs in the Supplement). As a result, with probability at least $1-\delta$, we find $h(n,\gamma,T,\delta)$ as follows:
\begin{equation*}
\begin{split}
\mathcal{R} \!&= \!\Pp_S\!\left(\mathscr{C}(\hat{Y})_s \!\in \! \left[e^{-T}, 1 \! - \! e^{-T}\right]\right) \!\!
\overbrace{\le}^{\text{T}\ref{thm:confidence_bounded}}\Pp_S\left(\psi_n \in [t_1, t_2] \right) \\
&= F_{\psi_n}(t_2) - F_{\psi_n}(t_1) \overbrace{\le}^{\text{T}\ref{thm:empirical_tau}} F_{\psi}(t_2) - F_{\psi}(t_1) + 2\sqrt{\frac{\ln{\frac{2}{\delta}}}{2n}}\\
&\!\!\overbrace{=}^{\text{T}\ref{thm:tau_is_uniform}} t_2(n,\gamma,T)\! -\! t_1(n,\gamma,T) \!+\! 2\sqrt{\frac{\ln{\frac{2}{\delta}}}{2n}} = h(n,\gamma,T,\delta).
\end{split}
\end{equation*}
\end{proof}

\paragraph{R2. Estimating the rejection rate.}
We estimate the rejection rate at the test time by measuring how many training examples would be rejected. This assumes that the test scores follow the same distribution as the training scores.
\begin{theorem}\label{thm:expected_rejection_rate}
Given $s \sim S$, let $g \colon [0,1] \to [0,1]$ be the function that maps $\psi_n \in [0,1]$, i.e. the proportion of training scores lower than $s$, to the confidence value $\mathscr{C}(\hat{Y})_s = g(\psi_n)$. Then, for high $n$ and $T\ge 4$, the rejection rate estimate $\hat{\mathcal{R}}$ approximates the true rejection rate $\mathcal{R}$
\begin{equation}
\hat{\mathcal{R}}= \hat{F}_{\psi_n}\left(g^{-1}\left(1-e^{-T}\right)\right) - \hat{F}_{\psi_n}\left(g^{-1}\left(e^{-T}\right)\right) \approx \mathcal{R}
\end{equation}
where $g^{-1}$ is the inverse-image through $g$, and $\hat{F}_{\psi_n}(u) = \Pp_{S_{tr}}(\psi_n \le u)$ for $u\in [0,1]$.
\end{theorem}
\begin{proof}
From the definition~\ref{defn:rejection_rate} and Theorem~\ref{thm:tau_is_uniform},
\begin{equation*}
\begin{split}
\mathcal{R} &= \Pp_S\left(\mathscr{C}(\hat{Y})_s \in \left[e^{-T}, 1- e^{-T}\right]\right) \\
&\approx \Pp_{S_{tr}}\left(g(\psi_n) \in \left[e^{-T}, 1- e^{-T}\right]\right)\\
&= \Pp_{S_{tr}}\left(\psi_n \in \left[g^{-1}\left(e^{-T}\right), g^{-1}\left(1- e^{-T}\right)\right]\right)\\
&= \hat{F}_{\psi_n}\left(g^{-1}\left(1-e^{-T}\right)\right) - \hat{F}_{\psi_n}\left(g^{-1}\left(e^{-T}\right)\right) = \hat{\mathcal{R}},
\end{split}
\end{equation*}
where the higher $n$ the closer the training distribution $S_{tr}$ to the theoretical score distribution $S$.
\end{proof}

\paragraph{R3. Bounding the expected cost.}
Using a reject option should theoretically help keep the total cost down. We estimate the upper bound by using that (1) the detector predicts on expectation $\gamma$ positive predictions, and (2) we have knowledge of the expected rejection rate.
\begin{theorem}\label{thm:cost_upperbound}
Let $c$ be a cost function as defined in Section~\ref{sec:preliminaries}, with $c_{fp}>0$, $c_{fn}>0$, and $c_r>0$ as costs for false positives, false negatives, and rejections. Let $g$ be as in Theorem~\ref{thm:expected_rejection_rate}. Given a (test) dataset $D_{te}$ such that $S_{te} = \{f(x_i)\}_{x_i\in D_{te}}$, and $T\ge 4$, the expected example-wise cost is bounded by
\begin{equation}
\E_{D_{te}}[c] \le \min\{\gamma, A\} c_{fn} + (1-B)c_{fp} + (B-A) c_r,
\end{equation}
where $A = \hat{F}_{\psi_n}(g^{-1}\left(e^{-T}\right))$, $B = \hat{F}_{\psi_n}(g^{-1}\left(1-e^{-T}\right))$, are as in Theorem~\ref{thm:expected_rejection_rate}.
\end{theorem}
\begin{proof}
Using Theorem~\ref{thm:expected_rejection_rate}, and indicating the non-rejected false positives and false negatives as, respectively, 
$$FP = \Pp(\hat{Y}=1|Y=0, \mathscr{C}(\hat{Y})_s > 1-\exp(-T))$$
$$FN = \Pp(\hat{Y}=0|Y=1, \mathscr{C}(\hat{Y})_s > 1-\exp(-T))$$
it follows that
\begin{equation*}
\begin{split}
\E_{D_{te}}[c] &= \E_{D_{te}}[c_{fn} FN + c_{fp} FP +c_r \mathcal{R}]\\
&= \E_{D_{te}}[c_{fn}FN] + \E_{D_{te}}[c_{fp}FP] + c_{r}(B-A)
\end{split}
\end{equation*}
where $A = \hat{F}_{\psi_n}(g^{-1}\left(e^{-T}\right))$, $B= \hat{F}_{\psi_n}(g^{-1}\left(1-e^{-T}\right))$ come from Theorem~\ref{thm:expected_rejection_rate}.
Now we observe that
\begin{itemize}
    \item $FP \le \Pp(\hat{Y}=1|\mathscr{C}(\hat{Y})_s > 1-\exp(-T)) = 1-B$ as you cannot have more false positives than accepted positive predictions;
    \item $FN \le \Pp(Y=1) = \gamma$ and $FN \le \Pp(\hat{Y}=0|\mathscr{C}(\hat{Y})_s > 1-\exp(-T)) = A$, as you can have more false negatives neither than actual positives ($\gamma$), nor than accepted negative predictions ($A$).
\end{itemize}
From these observations, we conclude that
\begin{equation*}
\E_{D_{te}}[c] \le \min\{\gamma, A\} c_{fn} +(1-B) c_{fp} + (B - A) c_r.
\end{equation*}
\end{proof}









%\begin{definition}[Rejection rate estimate]\label{defn: rejection_rate_estimate}
%Let $T>0$ be a positive constant. We define the rejection rate estimate as
%\begin{equation*}
%\hat{\mathcal{R}} \coloneqq \Pp\left(\mathscr{C}(\hat{Y})_x \in \left[e^{-T}, 1- e^{-T}\right]\right).
%\end{equation*}
%Note that, differently from definition~\ref{defn:rejection_rate}, the estimator does not include confidence values lower than $\exp(-T)$. 
%\end{definition}

%\begin{remark}
%As extremely low confidence values are unlikely to occur (see Theorem~\ref{thm:confidence_bounded}), the estimator $\hat{\mathcal{R}}$ is either slightly greater or approximately the same as the true rejection rate $\hat{\mathcal{R}} \gtrapprox \mathcal{R}$.
%\end{remark}
